Responsible AI (RAI) Games and Ensembles

Several recent works have studied the societal effects of AI; these include issues such as fairness, robustness, and safety. In many of these objectives, a learner seeks to minimize its worst-case loss over a set of predefined distributions (known as uncertainty sets), with usual examples being perturbed versions of the empirical distribution. In other words, aforementioned problems can be written as min-max problems over these uncertainty sets. In this work, we provide a general framework for studying these problems, which we refer to as Responsible AI (RAI) games. We provide two classes of algorithms for solving these games: (a) game-play based algorithms, and (b) greedy stagewise estimation algorithms. The former class is motivated by online learning and game theory, whereas the latter class is motivated by the classical statistical literature on boosting, and regression. We empirically demonstrate the applicability and competitive performance of our techniques for solving several RAI problems, particularly around subpopulation shift.

==> alt_bounds.tex <==
These bounds can be quite loose in practice. Specifically, for the binary case, if $\widehat{R}_W(\hrand) \leq \frac{1}{2}$ then we have $\widehat{R}_W(\hdet) = 0$. To this end, prior work \citet{lacasse2006pac, germain2015risk, masegosa2020second} has developed tighter bounds using second-order inequalities. 
\begin{proposition}
    Consider the setting with the zero-one loss $l(y', y) = \I[y' \neq y]$, and $\gamma_P$ defined as before. If $\widehat{R}_W(\hrand) \leq \frac{1}{\gamma_P}$ then,
    \begin{equation*}
        \widehat{R}_W(\hdet) \leq 2 \sup_{w \in W} e^{-\frac{2\l\frac{1}{\gamma_P} - \E_w\E_{P}\I[h(x) \neq y]\r^2}{Var_w(\E_P\I[h(x)\neq y])}} \leq 2 e^{-2\l\frac{1}{\gamma_P} - \widehat{R}_W(\hrand)\r^2}
    \end{equation*}
\end{proposition}
\begin{proof}
    \begin{align*}
    \widehat{R}_W(\hdet) = \sup_{w \in W} \E_w \ell(y_P(x),y) &\leq \sup_{w \in W} P_w(\E_{P}\I[h(x) \neq y] \geq 1/\gamma_P) \\
    &\leq 2\sup_{w \in W} e^{-\frac{2\l\frac{1}{\gamma_P} - \E_w\E_{P}\I[h(x) \neq y]\r^2}{Var_w(\E_P\I[h(x)\neq y])}} \text{\;\; $\l \E_w\E_{P}\I[h(x) \neq y] \leq \frac{1}{\gamma_P}\r$ (Hoeffding)}
\end{align*}
Also, we have $Var_w(\E_P\I[h(x)\neq y]) \leq 1$. Substituting this above completes the claim.
\end{proof}
\begin{remark}[Optimization]
    From above, we can also attempt optimizing the modified RAI game 
    \begin{align*}
        \inf_P \sup_{w} \frac{\l\frac{1}{\gamma_P} - \E_w\E_{P}\I[h(x) \neq y]\r^2}{Var_w(\E_P\I[h(x)\neq y])}
    \end{align*}
    From \citet{dinkelbach1967nonlinear}, we have if $f, g$ are quadratic functions with $g > 0$, then 
    \begin{align*}
        \min_{x \in S} \frac{f(x)}{g(x)} \leq \delta \iff \min_{x \in S} f(x) - \delta g(x) \le 0
    \end{align*}
    Thus, we can consider solving the game, for some $\alpha, \beta > 0$,
    \begin{align*}
        \inf_P \sup_w \l \E_w\E_P \I[h(x) \neq y] + \alpha \E_w (\E_P \I[h(x) \neq y])^2 - \beta (\E_w\E_P \I[h(x) \neq y])^2 \r
    \end{align*} As a special case, for $\beta =0$, this game is convex-concave and admits a NE.
\end{remark}

==> arxiv/review.tex <==
It does not have the general parameterization as well as the adaboost-esque greedy algorithm using general parameterization 
\begin{enumerate}
    \item The reason we care about this is that we can then perform adaboost-esque greedy algorithm which does not exactly solve the game (but could be motivated as solving a relaxation)
    \item The population section + generalization guarantees is kind of a mess. I have some thoughts on how to fix this, along lines of Schapiro.
    \item Experiments section also seems lackluster Note that boosting algorithms solve this game anyway, so why only compare to those? Also see first point above, it’s likely crucial to use the general greedy algorithm similar to adaboost, which at the very least has adaptive step sizes.
    \item Why not compare to novel intersections of sets 
\end{enumerate}
In overleaf I saw some comments on what was the point of the deterministic to randomized ensemble bounds. It’s actually a crucial motivation. Here is a restructuring of that section that should hopefully make it clear:
\begin{enumerate}
    \item After describing the RAI game, move the ensemble material to new section
    \item Start with a deterministic ensemble, and specify the deterministic ensemble RAI game
    \item This is computationally less amenable because of the non-smooth nature of the de-randomized predictions \item Contrast with a randomized ensemble Specify randomized ensembles, and randomized ensemble RAI game This can also be cast a linearization of RAI game, providing mixed strategies Easier to solve since essentially a bi-linear game
    \item Caveat: what we want is the deterministic ensemble rather than the randomized ensemble game 
    For zero-one loss, etc. we have a nice expression connecting deterministic and randomized RAI risk
    \item So, we can cast minimizing randomized RAI risk as minimizing an upper bound on deterministic ensemble RAI risk. Thus the corresponding randomized RAI game can be cast as a relaxation of the deterministic RAI game.
    \item  In the sequel, we thus focus on this randomized ensemble RAI game, which we will then use to obtain a deterministic ensemble. Following the bounds above, the corresponding deterministic ensemble risk will be bounded by the randomized ensemble RAI risk
\end{enumerate}

==> arxiv/trash.tex <==
    % Note that the constraint can be rewritten as $\{w: \vv{1}^Tw = 1, 0 \preccurlyeq w \preccurlyeq \frac{1}{\alpha n}\}$ which is an intersection of an affine constraint and a convex polytope and thus again a convex polytope.  Thus, optimization over a linear loss can be done by evaluating its vertices i.e. which are some linear combinations of our data points. The number of these should be polynomial in the number of constraints (for a fixed dimension). \\
    % The proof of Propositions $1, 2$ follows the same with the $n$ replaced with the number of vertices. \textcolor{red}{Arun: the proofs will go through for general sets $W$, but I don't think we need to replace $n$ with the number of vertices to get the rates. We can get something tighter. Even if we have smooth surfaces like spheres (which can viewed as having $\infty$ vertices), exponential weights algorithm will achieve good rates. Proposition 3 will also go through because FW converges for any bounded convex set $W$.}\\ {\color{blue} Can someone please verify this? Also, Proposition 3 would go through in this case as well, right?}
    % \item[]\textbf{Case-3} $W$ is an arbitrary convex set. \\
    % Proposition $1, 2$ again follow as we can use the Continuous Exponential Weights algorithm from Chapter 3 of ~\citep{bubeck2011introduction}. The RHS of Proposition $1$ becomes $\frac{\eta n log(1/\gamma)}{T} + \frac{1}{8\eta} + \gamma$ for any $\gamma > 0$. Here, $n$ is again the new effective data points. \\
    % {\color{blue} What about Proposition 3 here? Is the above correct? Is this new algorithm efficient? Page 23 of \citep{bubeck2011introduction} says random walk methods are efficient for convex bodies, but I am unsure. }


% \begin{algorithm}
%     \caption{General Recipe for RAI Games}
%     \label{alg-gen}
%     \begin{algorithmic}[1]\onehalfspacing
%         \Statex \textbf{Input:} Training data $\{(x_i, y_i)\}_{i=1}^n$, loss function $\ell$, constraint set $W$, hypothesis set $H$
%         \State \textbf{Initialize:} $w^0 \gets \frac{1}{n}[1,1,\dots 1]$, and $P^0 = 0$
%         \For{$t \gets 1$ to $T$}
%         \State $w^t \gets UPD_w(\{w^s\}_{s=0}^{t-1}, \{P^s\}_{s=0}^{t-1}, l, W)$
%         \State $P^t \gets UPD_P(\{w^s\}_{s=0}^{t}, \{P^s\}_{s=0}^{t-1}, l, H)$
%         \EndFor
%         \State \Return $w_T = AGG_w(\{w^t\}_{t=1}^T)$, $P_T = AGG_P(\{P^t\}_{t=1}^T)$
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
%     \caption{Entropic FTRL + BR}
%     \label{alg-1}
%     \begin{algorithmic}[1]\onehalfspacing
%         \Statex \textbf{Input:} Step length $\eta_t$, strongly-concave  regularizer $R$
%         % \For{$t \gets 1$ to $T$}
%         \State $UPD_w(*) = \arg\max_{w \in W} \left\{\sum_{s=1}^{t-1} \langle l^s, w \rangle + \eta_t R(w)\right\}$ \Comment{$l^s_i = l(h^s(x_i), y_i)$}
%         \State $h^s \gets \arg\min_{h \in H} \left\{\E_{(x, y) \sim w^t}[\ell(h(x), y)] \right\}$
%         \State $UPD_P(*) = P^{t-1} + h^s$
%         % \EndFor
%         \State \Return $w_T = \frac{1}{T} \sum_t w^t$, $P_T = Uniform(\{h^t\}_{t=1}^T)$
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
%     \caption{Sketch}
%     \label{alg-md}
%     \begin{algorithmic}[1]
%         \Statex \textbf{Input:} Training data $\{(x_i, y_i)\}_{i=1}^n$, step length $\eta_t$, strongly-concave  regularizer $R$, loss function $l$, $W$, $H$
%         \State $w^0 \sim Uniform(\{x_i, y_i\})$, $\upsilon^0 \sim $
%         \For{$t \gets 1$ to $T$}
%         \State $y^t \gets \nabla R^*(R(w^{t-1}) - \eta_t l^{t}) $ \Comment{$l^s_i = l(h^s(x_i), y_i)$}
%         \State $w^t \gets \Pi^R_W (y^t) $
%         \State $\upsilon^t \gets $
%         \EndFor
%         \State \Return $w_T = \frac{1}{T} \sum_t w^t$, $\upsilon_T = \frac{1}{T} \sum_t \upsilon^t$, $P_T = \{h_\theta\}_{\theta \sim \upsilon_T}$
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
%     \caption{Entropic FTRL + Frank Wolfe}
%     \label{alg-fw}
%     \begin{algorithmic}[1]\onehalfspacing
%         \Statex \textbf{Input:} Step length $\eta_t$, strongly-concave  regularizer $R$
%         \State $UPD_w(*) = \arg\max_{w \in W} \left\{\sum_{s=1}^{t-1} \alpha^s \langle l^s, w \rangle + \eta_t R(w)\right\}$ \Comment{$l^s_i = l(h^s(x_i), y_i)$}
%         \State $h^t \gets \arg\min_{h \in H} \langle \nabla_{P} L(P^{t-1}), h \rangle$ \Comment{$L(P) = \sum_{s=1}^{t-1} \alpha^s \langle l^s, w^t \rangle + \eta_t R(w^t)$}
%         \State $\alpha^t \gets \argmin_{\alpha \in [0,1]}  L((1-\alpha)P^{t-1} + \alpha h^t)$
%         \State $UPD_P(*) = (1-\alpha)P^{t-1} + \alpha h^t$
%         \State \Return $w_T = \frac{1}{T} \sum_t w^t$, $P_T = \sum_t \alpha^t h^t$
%     \end{algorithmic}
% \end{algorithm}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> mirror-descent-alg.tex <==
    \textbf{Remark}: Instead of iterating over $h_t$, can we directly update $P_t$? 
    We note that we can rewrite the game as a bilinear objective as,
    \begin{align*}
    \inf_{P \in \Delta_H} \sup_{w \in W} \langle w, AP \rangle
\end{align*} where $A: \Delta_H \rightarrow \mathcal{F}(X)$ is a linear operator (in possibly infinite dimension) defined as $(AP)(x) = \E_{h \sim P} [l(h(x), y)]$. 
Let's say our $h$ is parametrized as $h_\theta$ by some $\theta \sim \upsilon$. The game becomes
    \begin{align*}
        \min_{v \in V} \max_{w \in W} \E_{\theta \sim \upsilon, (x, y) \sim w} l(h_\theta(x), y) = \min_{v \in V} \max_{w \in W} \langle w, A \upsilon \rangle
    \end{align*} as before. Note that for linear operator $A$,
    \begin{align*}
        (Av)((x, y)) &= \E_{\theta \sim v} l(h_\theta (x), y) \\
        (A^\dagger w)(\theta) &= \E_{(x, y) \sim w} l(h_\theta(x), y)
    \end{align*}
    We want to iterate over $w, \upsilon$. The updates for online mirror descent are given as :
    \begin{align*}
        u^{t+1} &= \nabla R^*(\nabla R(u^t) + \eta A \upsilon^t),\; w^{t+1} = \Pi_W^R(u^{t+1})\\
        z^{t+1} &= \nabla R^*(\nabla R(z^t) - \eta A^\dagger w^t), v^{t+1} = \Pi_V^R(z^{t+1}) \\
    \end{align*}
    When $R$ is negative entropy,
    \begin{align*}
        u^{t+1}_i \propto \exp{(\eta Av^t((x_i, y_i)))} &= \exp{(\eta \E_{\theta\sim v^t}[l(h_\theta(x_i), y_i)])} \\
        z^{t+1}_\theta \propto \exp{(-\eta A^\dagger w^t(\theta))} &= \exp{(-\eta\E_{(x, y)\sim w^t}[l(h_\theta(x), y)])}
    \end{align*}
    The alternate version (where we use $w^{t+1}$) should be faster \citet{hsieh2021adaptive}? Can we compute this by sampling or other methods \cite{pmlr-v97-hsieh19b}? Can we de-randomize over this meaningfully? 

